Graph Filters for Signal Processing and Machine Learning on Graphs

Filters are fundamental in extracting information from data. For time series and image data that reside on Euclidean domains, filters are the crux of many signal processing and machine learning techniques, including convolutional neural networks. Increasingly, modern data also reside on networks and other irregular domains whose structure is better captured by a graph. To process and learn from such data, graph filters account for the structure of the underlying data domain. In this article, we provide a comprehensive overview of graph filters, including the different filtering categories, design strategies for each type, and trade-offs between different types of graph filters. We discuss how to extend graph filters into filter banks and graph neural networks to enhance the representational power; that is, to model a broader variety of signal classes, data patterns, and relationships. We also showcase the fundamental role of graph filters in signal processing and machine learning applications. Our aim is that this article provides a unifying framework for both beginner and experienced researchers, as well as a common understanding that promotes collaborations at the intersections of signal processing, machine learning, and application domains.

==> figures/freqResponse/freqResponse1.tex <==
%!TEX root = ../../00-groupMeetingLQR.tex

\def \thisplotscale {3.68}
\def \unit {\thisplotscale cm}

\def \frequencyresponse 
     {   0.8*exp(-(1*(x-1.2))^2) 
       + 0.7*exp(-(0.7*(x-4))^2) 
       + 0.8*exp(-(1.1*(x-6))^2) 
       + 0.1}

\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 1*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {0, 2.63, 6.72},
             xticklabels = {{\color{figBaseColor}$\lambda_1\phantom{\hat{\lambda}}$}, 
                            {\color{figBaseColor}$\lambda_i\phantom{\hat{\lambda}}$}, 
                            {\color{figBaseColor}$\lambda_{N}\phantom{\hat{\lambda}}$}},
             ymin = -0, ymax = 1.15,
             ytick = {-1},
             enlarge x limits=false]

\addplot+[samples at = {0.00, 0.91, 1.57, 
                        2.63, 3.97, 4.51, 
                        5.60, 6.72}, 
          color = figBaseColor, 
          ycomb, 
          mark=otimes*, 
          mark options={figBaseColor}]
         {\frequencyresponse};


\addplot[ domain=-0.5:7.5, 
          samples = 80, 
          color = black,
          line width = 0.8]
         {\frequencyresponse};


\end{axis}
\end{tikzpicture}


%{-0.22, 0.25, 0.61, 1.05, 1.37, 2.11, 
%  2.43, 3.07, 3.67, 4.13, 4.31, 5.05, 
%  5.20, 6.00, 6.42, 7.00}



==> figures/freqResponse/freqResponse2.tex <==
%!TEX root = ../../00-groupMeetingLQR.tex

\def \thisplotscale {3.68}
\def \unit {\thisplotscale cm}

\def \frequencyresponse 
     {   0.8*exp(-(1*(x-1.2))^2) 
       + 0.7*exp(-(0.7*(x-4))^2) 
       + 0.8*exp(-(1.1*(x-6))^2) 
       + 0.1}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 1*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {0.45, 3.37, 7.20},
             xticklabels = {{\color{figHighlightColor}$\hat{\lambda}_1$}, 
                            {\color{figHighlightColor}$\hat{\lambda}_i$},
                            {\color{figHighlightColor}$\hat{\lambda}_N$}},
             ymin = -0, ymax = 1.15,
             ytick = {-1},
             enlarge x limits=false]

\addplot+[samples at = {0.45, 1.25, 2.31, 
                        3.37, 4.23, 5.15, 
                        6.20, 7.20}, 
          color = figHighlightColor, 
          ycomb, 
          mark=oplus*, 
          mark options={figHighlightColor}]
         {\frequencyresponse};

\addplot[ domain=-0.5:7.5, 
          samples = 80, 
          color = black,
          line width = 0.8]
         {\frequencyresponse};


\end{axis}
\end{tikzpicture}


%{-0.22, 0.25, 0.61, 1.05, 1.37, 2.11, 
%  2.43, 3.07, 3.67, 4.13, 4.31, 5.05, 
%  5.20, 6.00, 6.42, 7.00}



==> figures/freqResponse/freqResponseBoth.tex <==
%!TEX root = ../../00-groupMeetingLQR.tex

\def \thisplotscale {3.68}
\def \unit {\thisplotscale cm}

\def \frequencyresponse 
     {   0.8*exp(-(1*(x-1.2))^2) 
       + 0.7*exp(-(0.7*(x-4))^2) 
       + 0.8*exp(-(1.1*(x-6))^2) 
       + 0.1}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 1*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {0, 0.45, 2.63, 3.37, 6.72, 7.20},
             xticklabels = {{\color{figBaseColor}$\lambda_1\phantom{\hat{\lambda}}$}, 
                            {\color{figHighlightColor}$\hat{\lambda}_1$}, 
                            {\color{figBaseColor}$\lambda_i\phantom{\hat{\lambda}}$}, 
                            {\color{figHighlightColor}$\hat{\lambda}_i$},
                            {\color{figBaseColor}$\lambda_{N}\phantom{\hat{\lambda}}$},
                            {\color{figHighlightColor}$\hat{\lambda}_N$}},
             ymin = -0, ymax = 1.15,
             ytick = {-1},
             enlarge x limits=false]

\addplot+[samples at = {0.00, 0.91, 1.57, 
                        2.63, 3.97, 4.51, 
                        5.60, 6.72}, 
          color = figBaseColor, 
          ycomb, 
          mark=otimes*, 
          mark options={figBaseColor}]
         {\frequencyresponse};

\addplot+[samples at = {0.45, 1.25, 2.31, 
                        3.37, 4.23, 5.15, 
                        6.20, 7.20}, 
          color = figHighlightColor, 
          ycomb, 
          mark=oplus*, 
          mark options={figHighlightColor}]
         {\frequencyresponse};

\addplot[ domain=-0.5:7.5, 
          samples = 80, 
          color = black,
          line width = 0.8]
         {\frequencyresponse};


\end{axis}
\end{tikzpicture}


%{-0.22, 0.25, 0.61, 1.05, 1.37, 2.11, 
%  2.43, 3.07, 3.67, 4.13, 4.31, 5.05, 
%  5.20, 6.00, 6.42, 7.00}



==> figures/freqResponse/graphDilationStableBoth.tex <==
%!TEX root = ../../00-groupMeetingLQR.tex

\def \thisplotscale {3.68}
\def \unit {\thisplotscale cm}

\def \frequencyresponse 
     { 0.9 - 0.7*exp(-(0.7*(x-1.6))^2) }

\hspace{-2.9mm}
\begin{tikzpicture}[x = 1*\unit, y=1*\unit]

\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\path [fill=black!20, opacity = 0.5] 
              (\deltax - 0.001*\factorx - \shadeshift, 0.00) rectangle 
              (\deltax + 0.030*\factorx + \shadeshift, 1.00);
\path [fill=black!20, opacity = 0.5] 
              (\deltax + 3.393*\factorx - \shadeshift, 0.00) rectangle 
              (\deltax + 3.770*\factorx + \shadeshift, 1.00);
\path [fill=black!20, opacity = 0.5] 
              (\deltax + 6.048*\factorx - \shadeshift, 0.00) rectangle 
              (\deltax + 6.720*\factorx + \shadeshift, 1.00);

\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 1*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {0.03, -0.01, 3.77, 3.393, 6.72, 6.048},
             xticklabels = {{\color{figHighlightColor}$\qquad\hat{\lambda}_1\phantom{\lambda}$},
                            {\color{figBaseColor}$\lambda_1\ \ $}, 
                            {\color{figHighlightColor}$\quad\hat{\lambda}_i\phantom{\lambda}$}, 
                            {\color{figBaseColor}$\lambda_i$},
                            {\color{figHighlightColor}$\quad\hat{\lambda}_{N}\phantom{\lambda}$},
                            {\color{figBaseColor}$\lambda_N$}},
             ymin = -0, ymax = 1.15,
             ytick = {-1},
             enlarge x limits=false]

\addplot+[samples at = {0.03, 0.91, 1.57, 
                        2.63, 3.77, 4.51, 
                        5.60, 6.72}, 
          color = figHighlightColor, 
          ycomb, 
          mark=otimes*, 
          mark options={figHighlightColor}]
         {\frequencyresponse};

\addplot+[samples at = {-0.01, 0.819, 1.413, 
                        2.367, 3.393, 4.059, 
                        5.04, 6.048}, 
          color = figBaseColor, 
          ycomb, 
          mark=oplus*, 
          mark options={figBaseColor}]
         {\frequencyresponse};

\addplot[ domain=-0.5:7.5, 
          samples = 80, 
          color = black,
          line width = 0.8]
         {\frequencyresponse};


\end{axis}
\end{tikzpicture}


%{-0.22, 0.25, 0.61, 1.05, 1.37, 2.11, 
%  2.43, 3.07, 3.67, 4.13, 4.31, 5.05, 
%  5.20, 6.00, 6.42, 7.00}



==> figures/graphConv/my_tikz_defs.tex <==

% This is a global control on the scale of plots. The constant \myfactor can be defined inside of an individual picture. It is good practice to reset \myfactor to 1 after the end of the picture.
\def\myfactor{1.0}
\def\unit{\myfactor cm}


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\footnotesize},   % Write numbers in tiny font
              label style = {font=\footnotesize}, % Write axes labels in footnote size font
              title style = {font=\footnotesize},
            }

% Definition of a graph node without filled in color. 
% Controls the appearance of a node in a graph plot
\tikzstyle{empty node} = [ circle, 
                     draw = black,
                     text = black, 
                     minimum size = 0.8*\unit]


% Definition of a graph node. Controls the appearance of a node in a graph plot
\tikzstyle{node} = [ empty node, 
                     fill = blue!50,
                     draw = blue!50,
                     text = white]

\tikzstyle{blue node} = [ empty node, 
                         fill = blue!50,
                         draw = blue!50,
                         text = white]

\tikzstyle{red node} = [ empty node, 
                         fill = red!50,
                         draw = red!50,
                         text = white]

\tikzstyle{green node} = [ empty node, 
                         fill = mygreen!50,
                         draw = mygreen!50,
                         text = white]


\tikzstyle{black node} = [ empty node, 
                           fill = black!40,
                           draw = black!40,
                           text = white]

                         
% Definition of a graph signal dot value without filled in color.
% These are smaller than the nodes and do not allow for text.
% Controls the appearance of a graph signal dot value in a graph plot
\tikzstyle{empty dot} = [ circle, 
                           draw = black,
                           inner sep = 0pt,
                           anchor = center,
                           minimum size = 0.4*\unit]


% Definition of a graph signal dot value.
% Controls the appearance of a graph signal dot value in a graph plot
\tikzstyle{dot} = [ empty dot, 
                    fill = blue!50,
                    draw = blue!50]

\tikzstyle{blue dot} = [ empty dot, 
                         fill = blue!50,
                         draw = blue!50]

\tikzstyle{red dot} = [ empty dot, 
                        fill = red!50,
                        draw = red!50]

\tikzstyle{black dot} = [ empty dot, 
                          fill = black!50,
                          draw = black!50]


% Definition of graph edges. An edge is undirected and doesn't contain arrows. A directed edge has an arrow at the end and a double directed edge contains two arrows. The latter is to be used when we want to emphasize the double directivity.
\tikzstyle{edge}                 = [shorten >=1pt, shorten <=1pt]
\tikzstyle{directed edge}        = [edge, -stealth]
\tikzstyle{double directed edge} = [edge, stealth-stealth]
\tikzstyle{tight edge}                 = [shorten >=0pt, shorten <=0pt]


% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]

